LOTOS: Layer-wise Orthogonalization for Training Robust Ensembles

Transferability of adversarial examples is a well-known property that endangers all classification models, even those that are only accessible through black-box queries. Prior work has shown that an ensemble of models is more resilient to transferability: the probability that an adversarial example is effective against most models of the ensemble is low. Thus, most ongoing research focuses on improving ensemble diversity. Another line of prior work has shown that Lipschitz continuity of the models can make models more robust since it limits how a model's output changes with small input perturbations. In this paper, we study the effect of Lipschitz continuity on transferability rates. We show that although a lower Lipschitz constant increases the robustness of a single model, it is not as beneficial in training robust ensembles as it increases the transferability rate of adversarial examples across models in the ensemble. Therefore, we introduce LOTOS, a new training paradigm for ensembles, which counteracts this adverse effect. It does so by promoting orthogonality among the top-$k$ sub-spaces of the transformations of the corresponding affine layers of any pair of models in the ensemble. We theoretically show that $k$ does not need to be large for convolutional layers, which makes the computational overhead negligible. Through various experiments, we show LOTOS increases the robust accuracy of ensembles of ResNet-18 models by $6$ percentage points (p.p) against black-box attacks on CIFAR-10. It is also capable of combining with the robustness of prior state-of-the-art methods for training robust ensembles to enhance their robust accuracy by $10.7$ p.p.

==> contents/4_setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

In this section, we describe the setup for our experiments. 

\noindent{\bf Models.}

In our experiments on verifying the trade-off of robustness and transferability (\Cref{sec:tradeoff}) we used ensembles of ResNet18 models (which are the common models used by prior work on training robust ensembles~\cite{}). These models are also used for observing the effect of ensemble size (\Cref{sec:size}), value of $k$ (\Cref{sec:var-k}). For verifying the effectiveness of LOTOS in decreasing the transferability rate of black-box attacks we use ResNet18 models in two cases: one with the original models and one with the batch normalization layers removed, as the prior work has shown the difference in the adversarial robustness of these two cases, with the latter one being more protective~\cite{boroojeny2024spectrum}. To show the effectiveness of LOTOS when combined with the prior methods of training robust ensembles in~\Cref{subsec:prior}, in addition to the results for ResNet18 models we report the results for DLA models which are larger models with more number of parameters. In~\Cref{subsec:hetero}, to show the effectiveness of LOTOS in ensembles of heterogeneous models, we use ResNet18 and ResNet34 models, which have different numbers of layers and layer sizes.

\noindent{\bf Datasets.}
For our experiments, we have used CIFAR10 (which is used in prior works on training robust ensembles) and CIFAR100 which is a more difficult dataset for the classification task.

\noindent{\bf Attacks Considered.}
The adversarial attacks that we consider in this work are PGD-$50$ with $\epsilon = 0.04$ (referred to as $\delta$ in~\Cref{sec:motivation}).  


\noindent{\bf Compute Infrastructure:} \varun{gpu, os, memory, processor speed etc.}
